Temporal upscaling in micro magnetism via heterogeneous multiscale methods

We consider a multiscale strategy addressing the disparate scales in the Landau-Lifschitz equations in micro-magnetism. At the microscopic scale, the dynamics of magnetic moments are driven by a high frequency field. On the macroscopic scale we are interested in simulating the dynamics of the magnetisation without fully resolving the microscopic scales. The method follows the framework of heterogeneous multiscale methods and it has two main ingredients: a micro- and a macroscale model. The microscopic model is assumed to be known exactly whereas the macro model is incomplete as it lacks effective quantities. The two models use different temporal and spatial scales and effective parameter values for the macro model are computed on the fly, allowing for improved efficiency over traditional one-scale schemes. For the analysis, we consider a single spin under a high frequency field and show that effective quantities can be obtained accurately with step-sizes much larger than the size of the microscopic scales required to resolve the microscopic features. Numerical results both for a single magnetic particle as well as a chain of interacting magnetic particles are given to validate the theory.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Declare title and authors, without \thanks
\newcommand{\TheTitle}{Temporal Upscaling in Micro Magnetism Via Heterogeneous Multiscale Methods}
\newcommand{\TheAuthors}{D. Arjmand, S. Engblom, and G. Kreiss}

% Sets running headers as well as PDF title and authors
\headers{Multiscale Modeling in Micro Magnetism}{\TheAuthors}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{{\TheTitle}}

% Authors: full names plus addresses.
\author{
 Doghonay Arjmand \thanks{Division of Scientific Computing, Department of Information Technology, Uppsala University, 
    (\email{doghonay.arjmand@it.uu.se},\email{stefane@it.uu.se},\email{gunilla.kreiss@it.uu.se}).}%\url{http://www.imag.com/\string~ddoe/}).}
  \and
   Stefan Engblom\footnotemark[1]
  \and
  Gunilla Kreiss\footnotemark[1]
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

